Causal inference for social network formation

This paper develops a framework for identification, estimation, and inference on the causal mechanisms driving endogenous social network formation. Identification is challenging because of unobserved confounders and reverse causality; inference is complicated by questions of equilibrium and sampling. We leverage repeated observations of a network over time and random variation in initial ties to address challenges to causal identification. Our design-based approach sidesteps questions of sampling and asymptotics by treating both the set of nodes (individuals) and potential outcomes as non-random. We apply our approach to data from a large professional services firm, where new hires are randomly assigned to project teams within offices. We estimate the causal effect on tie formation of indirect ties, network degree, and local network density. Indirect ties have a strong and significant positive effect on tie formation, while the effects of degree and density are smaller and less robust.

==> Sections/A_proofs.tex <==
\section{Proofs}
\label{sec:proofs}

\begin{proof}[Proof of \autoref{lem:IPW}:]$\;$
    \begin{itemize}
      \item By the structural relationship and the exclusion restriction, 
      $$Y_{ij} \cdot \bs 1(D_{ij} = d) = Y_{ij}^d \cdot \bs 1(D_{ij} = d).$$
      \item By the support condition, $P(D_{ij} = d)>0$
      \item Because $Y_{ij}^d$ is a function of $f$,
      $$E\left[Y_{ij}^d \cdot \frac{\bs 1(D_{ij} = d)}{P(D_{ij} = d )}\Big|f \right] = Y_{ij}^d \cdot E\left[\frac{\bs 1(D_{ij} = d)}{P(D_{ij} = d )}\Big|f \right]$$
      \item By the randomization condition,
      $$E\left[\frac{\bs 1(D_{ij} = d)}{P(D_{ij} = d )}
      \Big|f \right] = 1.$$
    \end{itemize}
    The claim follows.
\end{proof}

\clearpage
\begin{proof}[Proof of \autoref{lem:equivariance}:]$\;$
    \begin{enumerate}
      \item By item 3 of \autoref{ass:networkmodel} and \autoref{ass:permutation}, $A^1$ is a uniform random draw from $\mathcal A = \{A_\pi:\; \pi \in \Pi\}$.
      
      \item By definition, $p_{\pi(i)\pi(j)}(d) = P(d_{\pi(i)\pi(j)}(A^1) = d)$.
      
      \item By equivariance, $d_{\pi(i)\pi(j)}(A^1) = d_{ij}(A^1_\pi)$.
      
      \item By assumption, $A^1$ is a uniform draw from $\mathcal A = \{A_\pi':\; \pi' \in \Pi\}$.
        The mapping from $A$ to $A_\pi$ is one-to-one on $\mathcal A$, because $\Pi$ is a group: $\pi\circ \pi' \in \Pi$ and $\pi^{-1}\circ\pi'$ in $\Pi$, and thus $A_{\pi \circ \pi'}, A_{\pi^{-1} \circ \pi'} \in \mathcal A$.
        It follows that $A^1_{\pi}$ is also a uniform  random draw from $\mathcal A$. 
      
      \item Therefore the distribution of $d_{ij}(A^1_\pi)$ is the same as the distribution of $d_{ij}(A^1)$. The first claim follows.
      
      \item The second claim follows because
       $P_{\pi(i)\pi(j)} = p_{\pi(i)\pi(j)}(D_{\pi(i)\pi(j)}) = p_{ij}(D_{\pi(i)\pi(j)}) \sim p_{ij}(D_{ij}) = P_{ij},$
       where the first equality holds by definition, the second equality uses the first claim (applied at $d = D_{\pi(i)\pi(j)}$), and the distributional step uses $D_{\pi(i)\pi(j)} \sim D_{ij}$.
    \end{enumerate}
    
\end{proof}

\begin{proof}[Proof of \autoref{prop:ipw}:]$\;$
    \begin{enumerate}
      \item By the first order condition for the least squares estimator,
      \bals
      \widehat \beta &=
      \left(\sum_{(i,j) \in \mathcal E} \frac{1}{P_{ij}} D_{ij} \cdot D_{ij}'\right)^{-1} \cdot \left(\sum_{(i,j) \in \mathcal E} \frac{1}{P_{ij}} Y_{ij} \cdot  D_{ij}\right).
      \eals
      
      
      \item Consider the second term of this expression. By the structural relationship and the exclusion restriction, we can rewrite
      $$
       \frac{Y_{ij}  \cdot  D_{ij}}{P_{ij}}  = \sum_d Y_{ij}^d  \cdot  d \cdot \frac{\bs 1(D_{ij} = d)}{P(D_{ij} = d)}.
      $$
     Therefore, because $Y_{ij}^d$ is a function of $f$, and by the randomization condition and support condition (as in \autoref{lem:IPW}),
      $$
      E\left[\frac{ Y_{ij}  \cdot  D_{ij}}{P_{ij}}\Big | f\right] = 
      \sum_d Y_{ij}^d  \cdot  d.
      $$
    
      \item Consider next the first term of the expression for $\widehat \beta$. By a similar argument as for the second term, for all $i,j$
      $$
      E\left[\frac{1}{P_{ij}}D_{ij} \cdot D_{ij}'\Big | f\right] = 
      \sum_d d  \cdot d'.
      $$
    
      \item By \autoref{lem:equivariance}, $\frac{1}{P_{ij}}D_{ij} \cdot D_{ij}'$ is replaced by $\frac{1}{P_{\pi(i)\pi(j)}} D_{\pi(i)\pi(j)} \cdot D_{\pi(i)\pi(j)}'$ when the network $A^1$ is replaced by $A^1_\pi$.
      By the invarance condition for $\mathcal E$ of \autoref{ass:permutation}, 
      $$\sum_{(i,j) \in \mathcal E} \frac{1}{P_{\pi(i)\pi(j)}} D_{\pi(i)\pi(j)} \cdot D_{\pi(i)\pi(j)}'
      = \sum_{(i,j) \in \pi(\mathcal E)} \frac{1}{P_{ij}} D_{ij} \cdot D_{ij}'
      =\sum_{(i,j) \in \mathcal E} \frac{1}{P_{ij}} D_{ij} \cdot D_{ij}',      
      $$
      where we denote $\pi(\mathcal E) = \{(\pi(i), \pi(j)): (i,j) \in \mathcal E\}$.
      This implies that  $\sum_{(i,j) \in \mathcal E} \frac{1}{P_{ij}} D_{ij} \cdot D_{ij}'$ is invariant under the permutations $\pi \in \Pi$ of $A$, and therefore non-random.


    
      \item It follows from the previous two items that
      $$
      \frac{1}{|\mathcal E|}\sum_{(i,j) \in \mathcal E} \frac{1}{P_{ij}}D_{ij} \cdot D_{ij}' =
      \sum_d d  \cdot d'
      $$
      with probability $1$. The claim of the proposition follows, by collecting terms.
    \end{enumerate}
    
\end{proof}

\clearpage
\begin{proof}[Proof of \autoref{prop:withinregression}:]$\;$
  \begin{itemize}
  \item By the first order condition for the least squares estimator,
$$
\widehat \gamma_{j} =
\left(\sum_{i \in \mathcal I} D_{ij} \cdot D_{ij}'\right)^{-1} \cdot \left(\sum_{i \in \mathcal I} Y_{ij} \cdot D_{ij}\right).
$$

	\item By definition of $\mathcal{D}_{j}$,
$$
\left(\sum_{i \in \mathcal I} D_{ij} \cdot D_{ij}'\right) =\left(\sum_{d\in \mathcal D_{j}} d \cdot d'\right).
$$
By assumption, the right-hand side is invertible for all $j$.

\item By equivariance of $d_{ij}$ (\autoref{ass:permutation}), and because $\pi(j) = j$ for all $j \in \mathcal J$ and $\pi(\mathcal I) = \mathcal I$ (\autoref{ass:rectangular}), the set $\mathcal{D}_{j}$ is invariant under permutations. Therefore the right hand side is non-random.

	\item Consider next the second term in the expression for $\widehat{\gamma}_{j}$. By the structural relationship and the exclusion restriction, we can rewrite
	$Y_{ij} \cdot D_{ij} = Y_{ij}^{D_{ij}} \cdot D_{ij}$.
  

	\item By \autoref{ass:permutation}, by the assumed structure of $\Pi$ (\autoref{ass:rectangular}), and by the definition of $\mathcal{D}_{j}$, $D_{\pi(i)j}$ is a uniform draw from $\mathcal{D}_{j}$, and therefore the same holds for $D_{ij}$.
    Because $|\mathcal{D}_{j}|=|\mathcal{I}|$, we thus get
$$
E[Y_{ij}\cdot D_{ij} | f] = \frac{1}{|\mathcal{I}|} \sum_{d \in \mathcal{D}_{j}} Y_{ij}^{d}  \cdot d.
$$
The first claim of the proposition follows.

\item  Equality of $\gamma$ and $\beta$ is immediate from their definitions, if $\mathcal{D}_{j}=\mathcal{D}$.
\end{itemize}

\end{proof}


\begin{proof}[Proof of \autoref{prop:randomizationinference}:]$\;$
    Suppose that, under the null, the sampling distribution of $\widehat \beta$ is the same as the distribution of $\widehat \beta_\pi$, for a uniform draw of $\pi \in \Pi$. Under this assumption, the claim of the proposition follows.
    Under the null, $\widehat\beta$ is uniform over $\{\widehat\beta_\pi:\pi\in\Pi\}$; a permutation $\pi'$ satisfies $p_{\pi'}\leq\alpha$ iff at most $\alpha|\Pi|$ permutations give $\widehat\beta_\pi\geq\widehat\beta_{\pi'}$, and the number of such $\pi'$'s is at most $\lfloor\alpha|\Pi|\rfloor\leq\alpha|\Pi|$, so $P(p\leq\alpha)\leq\alpha$.\\

    It remains to show that our initial assumption was correct, so that the sampling distribution of $\widehat \beta$ is indeed the same as the distribution of $\widehat \beta_\pi$, for a uniform draw of $\pi \in \Pi$:
    \begin{enumerate}  
      \item  The group structure of $\Pi$ implies that  
      $$\mathcal A = \{A_\pi:\; \pi \in \Pi\} = \{A^1_\pi:\; \pi \in \Pi\}.$$
      We can therefore obtain the sampling distribution of $\widehat \beta$ by considering a uniform random draw of a permutation $\pi \in \Pi$, the counterfactual network $\tilde A^1 = A^1_\pi$, and the corresponding counterfactual realizations of $(\tilde D_{ij}, \tilde P_{ij}, \tilde Y_{ij})$, and calculating the corresponding counterfactual estimate $\tilde \beta$.
  
     \item  By equivariance (\autoref{ass:permutation}),
      the counterfactual $\tilde D_{ij}$ for the permutation $\pi$ satisfies
      $$
      \tilde D_{ij} = d_{ij}(A^1_{\pi}) = d_{\pi(i)\pi(j)}(A^1) = D_{\pi(i)\pi(j)}.
      $$
    
      \item  By \autoref{lem:equivariance}, the counterfactual $\tilde P_{ij}$ for the permutation $\pi$ satisfies
      $$
      \tilde P_{ij} =  p_{ij}(\tilde D_{ij}) =  p_{ij}(D_{\pi(i)\pi(j)}) = p_{\pi(i)\pi(j)}(D_{\pi(i)\pi(j)}) = P_{\pi(i)\pi(j)}.
      $$
    
      \item Under the null hypothesis, the counterfactual $\tilde Y_{ij}$ are the same as the realized $Y_{ij}$.
    
      \item Collecting the three preceding claims, we thus get that under the permutation $\pi$ of the entries of $A^1$, $(Y_{ij}, D_{ij}, P_{ij})$ is replaced by $(Y_{ij}, D_{\pi(i)\pi(j)}, P_{\pi(i)\pi(j)})$. 
      The counterfactual estimate $\tilde \beta$ is therefore equal to $\widehat \beta_\pi$, as defined in the statement of the proposition. 
      
      \item Since $\pi$ is a uniform random draw from $\Pi$, the claim follows.
    \end{enumerate}
  
 The claim for $\widehat \gamma$ and $\widehat \gamma_\pi$ follows by the same argument, once we note that under \autoref{ass:rectangular}, $d_{ij}(A_\pi) = D_{\pi(i)j}$, for $(i,j) \in \mathcal E$.
\end{proof}


\clearpage
\begin{proof}[Proof of \autoref{prop:standarderrors}:]$\;$
Denote $b_{o} = \frac{m_{o}}{m}\widehat{\beta}_{o}$, $\bar{b}_{o} = E[b_{o}|f]$, and $\epsilon_{o} = b_{o} - \bar{b}_{o}$.
Since $\widehat{\beta} = \sum_{o} b_{o} = \mathbf{1}'\mathbf{b}$, we have $\frac{m_{o}}{m}\widehat{\beta}_{o} - \frac{\widehat{\beta}}{N} = b_{o} - \frac{1}{N}\mathbf{1}'\mathbf{b} = (P\mathbf{b})_{o}$, where $P = I - \frac{1}{N}\mathbf{1}\mathbf{1}'$ is the $N\times N$ centering matrix. Hence
$$
\widehat{V}_{\beta} = \tfrac{N}{N-1}\,\mathbf{b}'P\mathbf{b}.
$$
Since $P$ is symmetric and idempotent ($P^{2}=P$), we can write
$$
\begin{aligned}
\tfrac{N-1}{N}\cdot E[\widehat{V}_{\beta}|f]
&= E[\mathbf{b}'P\mathbf{b}|f]\\
&= \bar{\mathbf{b}}'P\bar{\mathbf{b}} + E[\epsilon'P\epsilon|f]\\
&= \lVert P\bar{\mathbf{b}} \rVert^{2} + \operatorname{tr}(P\Sigma),
\end{aligned}
$$
where $\Sigma = \operatorname{diag}(\operatorname{Var}(\epsilon_{o}|f))$, using the independence of offices. Since $P_{oo} = 1 - \frac{1}{N} = \frac{N-1}{N}$ for all $o$, we have $\operatorname{tr}(P\Sigma) = \frac{N-1}{N}\sum_{o}\operatorname{Var}(\epsilon_{o}|f)$, and therefore
$$
E[\widehat{V}_{\beta}|f]
= \tfrac{N}{N-1}\lVert P\bar{\mathbf{b}} \rVert^{2} + \sum_{o}\operatorname{Var}\!\left(\tfrac{m_{o}}{m}\widehat{\beta}_{o}\,\big|\,f\right).
$$
By independence across offices, $\sigma_{\beta}^{2} = \operatorname{Var}(\widehat{\beta}|f) = \operatorname{Var}(\sum_{o} b_{o}|f) = \sum_{o}\operatorname{Var}(b_{o}|f)$.
Since $\lVert P\bar{\mathbf{b}} \rVert^{2} \geq 0$, it follows that $E[\widehat{V}_{\beta}|f] \geq \sigma_{\beta}^{2}$.
The claim for $\widehat{V}_{\gamma}$ follows by the same argument.
\end{proof}






==> Sections/B_additionalplots.tex <==
\section{Additional plots}
\label{sec:additionalplots}

\begin{figure}[H]
    \caption{Permutation distribution of placebo estimates}
    \label{fig:permutationplacebo}
\begin{center}
\vspace{10pt}


\includegraphics[width = \textwidth]{Figures_Tables/permutations_placebo_combined.pdf}\\[12pt]
\end{center}
\footnotesize
\textit{Notes:} These figures show the distribution of counterfactual estimates of placebo regressions under 10,000 permutations of new hires within offices. The black lines indicate the actual point estimate. The quantile of the point estimate in the randomization distribution corresponds to the p-values shown in \autoref{tab:placeboestimates}.
\end{figure}



\clearpage
\begin{figure}[H]
\caption{Permutation distribution of estimates}
\label{fig:permutationinference}
\vspace{10pt}
\includegraphics[width = \textwidth]{Figures_Tables/permutations_estimates_combined.pdf}\\[12pt]
\footnotesize
\textit{Notes:} These figures show the distribution of counterfactual estimates under 10,000 permutations of new hires within offices. The black lines indicate the actual point estimate. The quantile of the point estimate in the randomization distribution corresponds to the p-values shown in \autoref{tab:effectestimates}.\\[12pt]

\caption{Permutation distribution of estimates, continuous regressors}
\label{fig:permutationinferencecontinuous}
\vspace{10pt}
\includegraphics[width = \textwidth]{Figures_Tables/permutations_continuous_combined.pdf}\\[12pt]
\footnotesize
\textit{Notes:} These figures show the distribution of counterfactual estimates under 10,000 permutations of new hires within offices. The black lines indicate the actual point estimate. The quantile of the point estimate in the randomization distribution corresponds to the p-values shown in \autoref{tab:continuousestimates}.
\end{figure}





==> Sections/C_additionaldiscussion.tex <==
\section{Additional discussion}
\label{sec:additionaldiscussion}


\paragraph{Review: Causal inference in RCTs}
The framework as stated in \autoref{sec:setup} fairly abstract. To fix ideas and to motivate our estimands and estimators below, it is useful to relate this framework to the conventional setting of causal inference in randomized controlled trials with binary treatments \citep{imbens2015causal}.


This conventional setting describes the effect of binary treatments in the absence of interference (spillovers). There is a vector of outcomes $Y$, and a vector of treatments $D$, and the two are related by the causal relationship $Y = g(D)$.
The structural function $g$ (like the function $f$ in the network setting) describes potential (or counterfactual) outcomes. 
Under the assumption of {no interference} (also known as stable unit treatment effects, which is a form of {exclusion restriction}), $Y_j$ only depends on $D_j$, and it is common to define the {potential outcome} notation $Y^d_j = g(D_1,\ldots, D_{j-1}, d, D_{j+1},\ldots, D_n)$. 
A common object of interest is the {(sample) average treatment effect},
$$
SATE = \tfrac1n \sum_{j} \left(Y^1_j - Y^0_j\right).
$$
Note that this definition of the $SATE$ conditions on unobserved heterogeneity by conditioning on the function $g$.
The potential outcomes $Y^d_j$ are thus non-random, by definition; the only potential source of randomness is the treatment assignment $D$.



Under exogenous random assignment of $D$, the $SATE$ can be estimated without bias using {inverse probability weighting} (IPW).
We can write the IPW estimator of the SATE as follows:
\bals
  \widehat Y^d_j &= Y_j \cdot \frac{\bs 1(D_j = d)}{P(D_j = d)},
  &\widehat{SATE} &= \tfrac1n \sum_{j} \left(\widehat Y^1_j - \widehat Y^0_j\right).
\eals
Suppose that the {support condition} $0<P(D_j = 1)<1$ holds for all $j$.
Under this condition, it is easy to see that the IPW estimator is unbiased, $E\left[\widehat{SATE}\right] = SATE$.

We can furthermore perform {randomization inference} on $\widehat{SATE}$ and related objects: Randomization inference, for testing the null of zero treatment effects, assumes that $Y^1_j = Y^0_j$ for all $j$. Under the no interference condition and this null hypothesis, $g(D)$ is known for all counterfactual treatment assignments $D$. Because the sampling distribution of $D$ itself is known, the sampling distribution of any statistic based on $D$ and $Y$ is therefore known.

If heterogeneity or moderators of treatment effects are of interest, one might furthermore consider variants of the $SATE$ for subsets $\mathcal{I}$ of individuals $i$, where these subsets might be defined based on pre-determined individual covariates.

